Submerse: Visualizing Storm Surge Flooding Simulations in Immersive Display Ecologies

We present Submerse, an end-to-end framework for visualizing flooding scenarios on large and immersive display ecologies. Specifically, we reconstruct a surface mesh from input flood simulation data and generate a to-scale 3D virtual scene by incorporating geographical data such as terrain, textures, buildings, and additional scene objects. To optimize computation and memory performance for large simulation datasets, we discretize the data on an adaptive grid using dynamic quadtrees and support level-of-detail based rendering. Moreover, to provide a perception of flooding direction for a time instance, we animate the surface mesh by synthesizing water waves. As interaction is key for effective decision-making and analysis, we introduce two novel techniques for flood visualization in immersive systems: (1) an automatic scene-navigation method using optimal camera viewpoints generated for marked points-of-interest based on the display layout, and (2) an AR-based focus+context technique using an auxiliary display system. Submerse is developed in collaboration between computer scientists and atmospheric scientists. We evaluate the effectiveness of our system and application by conducting workshops with emergency managers, domain experts, and concerned stakeholders in the Stony Brook Reality Deck, an immersive gigapixel facility, to visualize a superstorm flooding scenario in New York City.

==> JosefCaseStudy.tex <==
 % \subsection{Expert Feedback}
% While forecasts for weather events have gotten more accurate over time, people's understanding of severe weather has not improved as much. With an increase in extreme weather events, such as hurricanes, and higher population densities near coasts, more people are exposed and vulnerable to loss of life and property damage when storms hit. The best way to prevent this loss is through preparations and evacuations. If a hurricane is forecasted to hit a particular area, such as New York City, meteorologists can use weather models to predicts potential impacts, such as storm surge. Currently, the National Hurricane Center puts out 2D maps of potential water depths in impacted areas. Here, the ability to more finely see and explore such data, especially in a 3D immersive setting is very helpful. The translation of a numerical water value to a 3D display, where users can see predicted water depths on buildings, is more effective than trying to interpret that information from colors. This can aid in decision making for individual stakeholders as well as emergency managers. People can see where to expect the worst impacts and where to focus preparations and evacuations. While meteorologists may have a better idea of the impacts of severe weather based on numerical data, visualizing weather impact data helps everyone's understanding. The high resolution display also helps users to get down to a more local level than the National Hurricane Center maps can display, further aiding in show places that are more vulnerable and important to users. In addition, meteorologists use ensemble forecasts using multiple model runs with slight differences to obtain a better and bigger envelope of possibilities. An immersive 3D display would also aid in show this envelope of possibilities, better communicating the uncertainties in the forecast than traditional methods. 
    
    


\subsection{Case Studies}
%-EM Workshop
	The technologies described in this paper were implemented in a workshop involving Emergency Managers, NOAA officials, and faculty to gauge their usefulness. Their feedback supported the notion that this type of display would aid in their work, with being able to focus on the most vulnerable areas in a most likely or worst case scenario of flooding. Participants also said that they would like the ability to have demographic information, critical facilities information, and vulnerable population data, which would now be achieved using the auxiliary display. Overall, the participants liked the experience and couuld envision how it would be helpful for their work.
	
%-College students workshop
	Storm surge flooding visualizations were also used in a separate workshop where college students were exposed to the storm surge visualizations. The workshop looked to see how these visualizations affected students' decision making. The participants agreed that the visualizations aided their decision making. The ability to "see" the flooding that could happen before it happened made participants more likely to avoid that situation. Visualizing storm surge flooding was more effective and improved their understanding rather than a numerical forecast of water depth, such as "We are expecting 3-5 feet of storm surge flooding." Just a numerical value is abstract to may people, but seeing water depth is more helpful. Some of the feedback received was that the color of the water was important to these types of stakeholders, as blue water looks more inviting and less scary than brown or murky water would have. 

%-Met club viewing
    A group of atmospheric science students were also brought in to give their feedback on the technologies. The students imagined that the display would greatly help with learning capabilities, especially in a meteorological sense. Phenomena in atmospheric science are 4 dimensional, covering a horizontal breadth, vertical height, and evolving over time. Being immersed in such a phenomena in 3D and seeing it evolve over time would aid in student learning, as compared to traditional 2D diagrams. The students also said that the display would be useful to display atmospheric model data in 3D, rather than the conventional 2D model outputs. They also said that the display of flooding in 3D with actual buildings was a much more effective method of communicating risks, rather than a numerical water depth forecast or a 2D flood risk map. 



\subsection{Comments/feasibility/advantages}
	The ability to use AR with the immersive tiled-display allows for users to look at the globally displayed data while being able to use AR to manipulate data locally without affecting the global display. This allows users to look at individually relevant points of interest while being in the same space, and with the backdrop of the global display. AR also enables users to see more information about specific points in the global data, such as water levels at specific buildings or areas. 
    Another advantage is that the Augmented Reality display can be used to visualize the uncertainty in forecasted flood heights, while maintaining the mean flood height in the global display. 



==> alg_path.tex <==

\begin{algorithm}[t]
 \caption{Camera viewpoints and navigation path generation}
\SetAlgoLined
\DontPrintSemicolon 
\KwIn{Display layout, POI list P, pitch threshold A, and distance threshold K }

$C \gets $ PSO($E$) \Comment{solve for Eq.~\ref{eq:optimization}} \;
$Q \gets \{\}$ \Comment{initialize empty set of POIs } \label{test}\; 
\ForEach{$p \in P$}{
obtain $c \in C$ that contains $p$ in its view \;
\uIf{$|c_{xyz}-p_{xyz}| > K $ \textbf{or} $c_{pitch} > A$} \;
{
$Q \gets p$ \;
\lIf{only $p$ in $c$}{ $C.remove(c)$ }\;
}
}

\end{algorithm}

\begin{algorithm}
\SetKwFor{For}{for (}{) $\lbrace$}{$\rbrace$ end for}
\caption{Camera path generation}
% \SetKwIF{If}{If (}{) $\lbrace$}{$\rbrace$}{}
\KwData{City's geographical data, user specification of the weights in viewpoint optimization, POI list (position, radius), Camera configuration}
\KwResult{Camera pose set $ C = \{ c_i \}$ }
$\text{Remaining list~} Q_{R} \gets{ POI~list } $\;
%$\text{overlapped curve list} \gets{\{\}} $\;
%{The objects are sorted based on the importance list in descending order}\;

Particle Swarm Optimization for { $p_{v_i}\in \{C\}$  }\;
    {
        \For{$o_i\in P_R$}{
        \text{Calculate} E_i (Equation~\ref{eq:overall_objective_function})\;
      
            If E_i < T:
        
            ~~~~~~Remove $o_i$ from $Q_R$\;
        
        Repeat PSO until $Q_R$ is \emptyset \;
        
    }
    \For{$c_i\in C$}
    {
    If no occlusion between $c_i$ and $c_{i+1}$:
    
    ~~~~~~Generate S_{Line}($c_i$, $c_{i+1}$)\;
    
    Else:
    
    ~~~~~~Generate S_{B\'{e}zier}($c_i$, $c_{i+1}$)\;
    }
}
    

% $\text{Select the optimal path based on Equation ~\ref{eqn:energy_function}.}$
\label{alg:pathGeneration}
\end{algorithm}

==> data_update.tex <==

The time to retrieve data in quadtrees increases with growing tree depth due to the large spatial extents of the data.
More so, it becomes redundant for a display node to construct a quadtree with spatial extents that span far beyond its camera viewing frustum.
As interactivity is critical, we limit the spatial bounds of the quadtree to enable efficient-time quadtree traversal.
For each defined screen, first, the camera projection matrix is determined based on the screen's relative position from the \textit{head} and the defined camera parameters.
Using the projection matrix, the bounds of the quadtree for the physical screen are defined such that the screen is positioned at the center of the entire quadtree, and the quadtree is scaled to cover the maximum horizontal extents of the camera-view frustum pyramid $+$ buffer size.
ADD FIG.XX.

Moreover, to maintain an interactive framerate for virtual exploration of the scene, we have designed a dynamic quadtree whose quadrants are updated based on the direction of the camera movement. 
Essentially, we allow the spatial extents of the quadtree, that is, the spatial bounds of the quadtree root, to be dynamic.
By tracking the displacement of the physical screen in the virtual scene, we are able to update the spatial bounds of the root when the screen approaches close to the outer boundary of one of its children.
Consequently, instead of constructing an entire quadtree with new spatial extents, we discard the first-level quadnodes (that is, the children of the quadree root) that are beyond a threshold distance from the screen position, rearrange the quadrant pointers of the preserved nodes to reflect the new root bounds, and construct nodes for the new bound range.
ADD FIG XX.
In our implementation, the quadnode updates are performed in parallel using multi-threading and are either triggered as the user manually navigates through the virtual scene or scheduled sequentially based on a predefined camera path generated using our algorithm described in Sec.~\ref{sec:cam_view}.

==> disp_table.tex <==
\begin{table}
\label{tab:specs}
\centering
\caption{Display system specifications}
\begin{tabular}{|l|c|c|c|c|} 
\hline
\multicolumn{1}{|c|}{\begin{tabular}[c]{@{}c@{}}\textbf{Display }\\\textbf{System}\end{tabular}} & \begin{tabular}[c]{@{}c@{}}\textbf{Display}\\\textbf{screens}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{GPUs /}\\\textbf{~screen}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Dimensions / }\\\textbf{screen (m)}\end{tabular} & \begin{tabular}[c]{@{}c@{}}\textbf{Horizontal}\\\textbf{FoV (\textdegree)}\end{tabular} \\ 
\hline
Desktop  & 1 & 1 & 0.62 $\times$ 0.36 & 80 \\ 
\hline
Tiled-display & 2 & 1 & 1.86 $\times$ 0.36 & 120 \\ 
\hline
Reality Deck & 26 & 4 & 7.44 $\times$ 2.88 & 360 \\
\hline
\end{tabular}
\end{table}
